Do Reasoning Representations Help Humans Evaluate LLM Outputs?

Reasoning representations are increasingly used as explanations for large language model outputs. Yet they are typically evaluated with model-centric criteria, such as answer accuracy and faithfulness, leaving it unclear whether they help people evaluate model responses. In this work, we study reasoning representations as human-facing interfaces rather than proxies for model reasoning ability. We conduct a controlled human study of six reasoning formats across tasks of varying complexity, supported by a web-based framework that randomizes task domains, problem instances, and representation order. The study collects fine-grained judgments of structural understanding, error detection and localization, and trust calibration. Our study shows a mismatch between perceived preference and support for human evaluation. Participants prefer planning- and decomposition-based representations, but simpler chain-of-thought traces better support verification, trust, and interpretability. Preferred representations also introduce calibration risks, with more false alarms on correct traces and high trust despite low willingness to verify.

==> sections/6_discussion.tex <==
\section{Discussion}
\label{sec:discussion}

\SH{Implications for Reasoning Representation Design}

Our results indicate that representation choice fundamentally shapes users’ ability to inspect LLM reasoning. Even when interaction is available, representations that preserve step-centric chain-of-thought can limit verification and comparison. By contrast, task-driven primitives make reasoning elements explicit and relationships traceable.




